ID.8: Co-Creating Visual Stories with Generative AI

Storytelling is an integral part of human culture and significantly impacts cognitive and socio-emotional development and connection. Despite the importance of interactive visual storytelling, the process of creating such content requires specialized skills and is labor-intensive. This paper introduces ID.8, an open-source system designed for the co-creation of visual stories with generative AI. We focus on enabling an inclusive storytelling experience by simplifying the content creation process and allowing for customization. Our user evaluation confirms a generally positive user experience in domains such as enjoyment and exploration, while highlighting areas for improvement, particularly in immersiveness, alignment, and partnership between the user and the AI system. Overall, our findings indicate promising possibilities for empowering people to create visual stories with generative AI. This work contributes a novel content authoring system, ID.8, and insights into the challenges and potential of using generative AI for multimedia content creation.

==> dummy.tex <==
\section{Evaluation Methodology}

We carried out a series of user studies to assess the usability of our platform and to explore the practicality of incorporating generative AI into a visual story co-creation system. Our evaluation methods included an in-lab usability test, a short-term longitudinal study of system deployment in-the-wild, a comparative case study to understand the pros and cons of traditional hand-crafted methods against our human-AI collaborative approach of visual story authoring, and an analysis of children's reactions to a selection of stories generated through our system.

%G created a story set in an enchanted forest, where three 'Ninja Princesses' are the guardians of their kingdom. Their idyllic life is disrupted when an evil Warlock Wolf steals a magical crown with the power to destroy their realm. Through a journey of bravery and skill, the princesses defeat the wolf, who ultimately shows remorse, and they restore peace to their kingdom.
%M crafted a tale set in the magical kingdom of Eldoria, where Sir Oliver, a dragon-riding knight, and his golden dragon, Ember, embark on a quest to defeat a fearsome dark beast terrorizing the kingdom. With the aid of magical creatures and a fairy-given arrow, they vanquish the beast and return as heroes, symbolizing the enduring power of courage and friendship.
%A \& Ma made a story about Ralph, a curious penguin in Penguin Bay who discovers a trove of beautiful seashells. Initially reluctant to share, Ralph eventually realizes the joy of generosity and community, transforming the bay's playground and learning that true happiness comes from making others smile.
%T created a story set in the Amazon rainforest, where a group of animals face the threat of deforestation. Banding together, they raise awareness through peaceful protests and outreach; It emphasizes the power of collective action and the importance of living in harmony with nature.
%M visualized a narrative about Alma, a young woman eager for quick gardening results. With the help of Jake, a savvy nursery worker, she selects Rainbow Snapdragons for her garden. Her work is rewarded as her garden swiftly bursts into a spectacle of vivid colors.


Stories play a critical role in the social, emotional, and cognitive development of children \cite{sugiyama2001narrative}. Engaging in storytelling and listening to stories leads to improved linguistic development by exposing them to a rich language environment with a rich array of new words, sentence structure, and complex syntax \cite{wells1986meaning}. Stories are also linked to improved critical thinking in children as they learn to understand cause and effect, make predictions, and solve problems presented in the plot. Similarly, storytelling may lead to enhanced empathy, imagination, creativity, interpersonal skills, and moral and ethical understanding. Stories can also be a means of coping or a mechanism for teaching coping techniques. Oral Stories, Books, Comics, Cartoons, Animations, and Video Games are just a few methods of story delivery for children. Multi-modal stories have been found to lead to better engagement and outcomes for children. 



Interactive visual stories can be an effective tool for children's learning and development as they lead to enhanced engagement and increased immersion, improved retention and comprehension, and opportunities for personalization and dynamic plotlines. Several interventions used interactive and visual stories as a platform to of delivering intervention content to children. Stories can help engage children in a wide variety of modalities -- collaborative storytelling \cite{dietz2021storycoder, dietz2023visual, rutta2020collaborative}, creative story creation \cite{zhang2022storydrawer}, and interactive stories \cite{michaelis2023off, michaelis2018reading} to name a few. Interactive visual stories can be delivered through embodied agents, both virtual and physical, social robots have been particularly effective in using storytelling as a medium to drive interactive sessions to deliver educational content \cite{bradlyn2003psychoeducational, scassellati2018improving, michaelis2018reading}. 

Despite the value of visual and interactive stories for children's development and learning, creating these kinds of stories takes a lot of effort and requires expertise in use of special software. Even creating the assets for these stories is a significantly time-consuming endeavor. There have been several efforts in simplifying the story creation process which has demonstrated the possibility of empowering non-experts with creating engaging stories; moreover, recent advancements in generative AI hold promise in democratizing asset creation. Allowing children to pick and choose from a diverse set of stories and interaction settings would make the storytelling experience more inclusive for a broader range of children.


\subsubsection{Open-Source ID.8}
We aim to open-source our system, first in the form of Docker containers and then in the form of an online platform that can help foster a community of creators and engineers around co-creating visual stories with the state-of-the-art generative AI. Beyond using our system to generate stories and intervention content, we hope our system may be used as a platform to better understand human-AI interaction and collaboration in the creative domain.

%Our Communication question (Q11) measures the user’s perception of the system’s ability to understand them, and the related Alignment
%Question (Q12) measures the efficacy of that communication in guiding the system towards their goals.

%Agency (Q13) question asks the inverse of the alignment question: whether the system was perceived as guiding the user towards its own goals. The Partnership question (Q14) makes the notion of collaboration vs tool use explicit by asking if the system and user were “collaborating as equals”. Perceiving human-machine collaboration as "equals" is an ambitious goal that is likely unfamiliar for most users, 

%The Contribution question (Q15) concerns the user and system’s agency: where does the user believe the locus of creative responsibility lies? The Satisfaction question (Q16) rates how happy they were with the output—a quality that may or may not be correlated with their overall enjoyment. The Surprise and Novelty questions (Q17 & Q18) ask participants to rate sketches along two dimensions traditionally associated with creative products but take care to avoid passing normative judgement in their phrasing.


 emphasizing the themes of courage and friendship. In G's story, three 'Ninja Princesses' in an enchanted forest defeat an evil Warlock Wolf to reclaim a stolen magical crown, ultimately restoring peace to their realm.  A \& Ma focus on Ralph, a penguin in Penguin Bay who discovers the beauty of sharing and community through distributing seashells. T spotlights current environmental concerns by setting a story in the Amazon rainforest where animals unite to fight deforestation through peaceful protests, emphasizing the importance of collective action and living in harmony with nature. Lastly, M tells the tale of Alma, a young woman who, with the help of a savvy nursery worker named Jake, selects Rainbow Snapdragons to swiftly turn her garden into a vivid spectacle.

%STUDY 1
%Breakdowns: Ease of creation dialogue between characters, automatic saving progress, segmentation, nudity/gore/bias in the image generation, generation time and need to generate multiple times, prompting difficulties, forgot how to duplicate scenes, forgot how to removing a sprite, unclear understanding of complex diffusion model terminology, sorted sprites, learning curve:  forgot how to connect nodes, slow, interminable content generation should timeout, too many storyboard, not auto-generated, editing scene, interaction [choices] creation

%Limitations: Speech bubbles functionality, Audio Generation Duration Limit, More animated character, screenplay breakdown/editing, generate the same character in different poses and clothes, sprited characters, Wanted to explore multiple different storylines, like dynamic plots, script simultaneously accessible, wanted more complex paths, chatbot didn’t work on the character development enough

%In terms of Enjoyment, Exploration, Expressiveness, Worth, and Alignment sub-scales of MICSI, median scores exceeded 5, confirming a predominantly positive user experience in these domains. These sentiments were also corroborated by the qualitative data from interviews. However, the scores for Immersiveness, Agency, and Partnership fell below 5, indicating areas where the user experience could be improved. The interview data reinforced these findings. Despite these lower scores, most users were pleased with the stories they co-created within the allocated time and felt that their contributions were equally matched by the system.


\subsubsection{Expanded Interactivity Opportunity}
Going beyond the shallow branching story based on user input that ID.8 currently supports may help expand the nature of stories that may be created using ID.8. Supporting further narrative decision-making 
with enabling alternative endings and word state choices may lead to improved engagement with the story and sense of agency in the viewer\cite{ligthart2020design}; Supporting more complex interactions such as backchanneling, co-reenactment, voice-based inputs may further enhance user engagement and expand the nature of content that is producible using ID.8. 

%\subsubsection{Embodied Story Delivery}
%Beyond just story content generation, the embodiment accompanying the content delivery has a significant impact on the perception of the viewer, 


% static story delivery, 
%Design Patterns for an Interactive Storytelling Robot to Support Children’s Engagement and Agency


\subsection{Overview and Workflow}
In ID.8, the process of creating a story is structured as a multi-stage workflow that combines human input and AI-generated content. Users initiate their project in the Storyline Creator module, where they work alongside GPT-3.5 Large Language Model alias 'Leela'. Here, users submit initial prompts or ideas, to which Leela responds by asking clarifying questions and making suggestions to help generate a narrative script which the user can edit to make more granular changes(Figure \ref{fig:sys-story-generation} (1)). This interaction allows users to focus on broader narrative elements such as themes and character development.
After the narrative has been formulated, it is systematically converted into a structured script using GPT3.5. This script is then used to pre-populate the Storyboard module with scenes with monochromatic backgrounds generated using StableDiffusion; Here, scenes are represented as individual nodes (Figure \ref{fig:sys-story-generation} (3)). The Storyboard serves as an organizational tool, offering a comprehensive view of the narrative structure. Users have the flexibility to rearrange, add, or delete scenes to alter the story's progression (Figure \ref{fig:sys-storyboard}). The Storyboard also includes an option for users to incorporate interactive elements at the end of scenes, such as questions aimed at the audience which may modify the flow of the story or be used to quiz viewers. This feature adds a layer of interactivity, giving viewers the opportunity to influence the direction of the story.

The next step involves the Scene Editor, a module that provides users with tools to further develop individual scenes by defining the various elements of each scene and their actions (e.g. characters, audio/music/speech, background etc) (Figure \ref{fig:sys-storyboard}). Using the Asset Creator inside Scene Editor, visuals (such as: backgrounds, characters) and audio (such as: background music, audio effect) can be generated or modified to align with the narrative content (Figure \ref{fig:sys-esset-generation}). This is facilitated by diffusion models specifically designed for text-to-image and text-to-audio conversions.

